A Systematic Approach to Blocking Convolutional Neural Networks

Convolutional Neural Networks (CNNs) are the state of the art solution for many computer vision problems, and many researchers have explored optimized implementations. Most implementations heuristically block the computation to deal with the large data sizes and high data reuse of CNNs. This paper explores how to block CNN computations for memory locality by creating an analytical model for CNN-like loop nests. Using this model we automatically derive optimized blockings for common networks that improve the energy efficiency of custom hardware implementations by up to an order of magnitude. Compared to traditional CNN CPU implementations based on highly-tuned, hand-optimized BLAS libraries,our x86 programs implementing the optimal blocking reduce the number of memory accesses by up to 90%.

==> Ack.tex <==
\section{Acknowledgement}
This work leverages Halide CNN code created by Ravi Teja Mullapudi~\cite{halideNN} to produce the performance result. Blaine Burton Rister has provided useful suggestions about the optimization algorithm and comments about paper writing.



==> old/Multi_core.tex <==
%\section{Multi-core Parallelism}
\section{Multi-core blocking choices}
\label{sec:Parallel}

1.	Model for estimate broadcast/wire energy, including data shuffling energy evaluation

2.	We choose two partition approaches, which are across kernel buffer and input buffer. How does the interconnection look like.


==> old/Notes.tex <==

{\color{red}
%\vspace{-\baselineskip}
%\noindent\hrulefill

\noindent {\large\bf TODO / NOTES}

\vspace{1\baselineskip}
\noindent 1a. Writing

\begin{itemize} \small
\item {\bf *** NO CONCLUSIONS (0\% done) ***}
\item Did we decide not to do old section 5 "multi-core blocking"?
\end{itemize}

\noindent 1b. Cleaning up
\begin{itemize} \small
\item Add fig for FC and CONV layers (see XY comment end of sec. 2.1)
\item Theory section refers to a missing ``eq:totalenergy" (see log)
\item Choose a format for Table 1
\item Add missing numbers to Table 1
\item Clean up section 2.3 (related work) (90\% done)
\item Clean up Sec. 3 "Theory" (70\% done)
\item Clean up Sec. 4 "Flex" (90\% done?)
\item Clean up Sec. 5 "methodology" (90\% done)
\item Clean up Sec. 6.1 "GP result" (85\% done)
\item Clean up Sec. 6.2 "custom result" (80\% done)
\item Finalize complete rough draft of paper.
\item Make sure paper compiles without errors
\end{itemize}

\noindent 2. Give paper to Mark for comments (nov 16)

\noindent 3. Address Mark comments

\noindent 4. Submit paper (nov 23)


\vspace{1\baselineskip}
\noindent ISCA Details
\begin{itemize} \small
\item ISCA submit deadline Nov. 23: %\newline
{\scriptsize
\url{isca2016.eecs.umich.edu/ index.php/2015/09/09/deadlines-for-isca-2016-announced/}}

\item
%10/15/2015 Double-checked to confirm that ISCA style file is the same as the MICRO style file we are currently using, also see
ISCA submission guidelines:\newline\indent
{ \scriptsize isca2016.eecs.umich.edu/index.php/submission/}

\item
{\it Papers ... should contain a maximum of 11 pages ... not including references.}

\end{itemize}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\ignore{
\vspace{\baselineskip}

\noindent {\bf ANSWERED / DONE}
\begin{itemize} \small
  \item \sout{
    Previously was using HY as abbrev for hybrid architecture. Should we change these to FIVA instead?
    Answer: Yes, change to FIVA.
  }
  \item \sout{
    Table~\ref{tab:opcounts} {\it (application complexity)} uses ``TSMC 45GS" technology while
    Table~\ref{tab:primitive_area} {\it (area of PS primitives)} uses ``40nm".  Is this consistent?  Should we use the same term for both?  Answer: both use TSMC 45GS.
  }
\end{itemize}
} %ignore

\ignore{{\noindent \normalsize\bf OUTLINE}
\vspace{-0.5\baselineskip}
\begin{small}
\begin{verbatim}
  1. Introduction
  2. OVERVIEW OF CNN / DNN PROBLEM
    2.1. The structure of the computation
    2.2. Current state of the art
    2.3. Realted work

  3. ANALYSIS APPROACH (SINGLE LAYER) FOR CONVOLUTIONAL 
  AND FULLY-CONNECTED (OLD STUFF)
    3.1 Motivation of blocking
    3.2 Trade-offs of blocking
    3.3 Terminology, and Analysis of Blocking
    3.4 Optimization Framework

  4. FLEXIBLE MEMORY DESIGN
  5. MULTI-CORE BLOCKING CHOICES
  6. METHODOLOGY
  7. EXPERIMENTAL RESULTS
    7.1  General processor result
      7.1.a. Single core
      7.1.b. Multi core
    7.2 Custom hardware result
      7.2.a. Single core
      7.2.b. Multi core

  8. Conclusion
\end{verbatim}
\end{small}
} %ignore
% \noindent\hrulefill
} %red


==> old/Related.tex <==
\subsection{Related Work}

(related)


==> old/Single_core.tex <==
%\section{CNN Core Design}
\section{Single core design space}
1.	CNN core architectural templates for conv/fully, pooling, LRU. describe the datapath, and register file (#ports, entry width).

2.	How to map a convolution, fully-connected layers to this core, what is the restriction on the scheduling. Pooling and LRU mapping are trivially done.

3.	How does memory hierarchy get changed? some buffers are flattened into the datapath. The register file implementation considerations (e.g. SRAM vs regfile, banks, ports, shift register design for some configs). 

4.	Efficiency analysis on the core design. How do different parameters affect the energy and area efficiency?

5.	Flexible architecture's energy overhead  

